Audio-based AI classifiers show no evidence of improved COVID-19 screening over simple symptoms checkers

Recent work has reported that AI classifiers trained on audio recordings can accurately predict severe acute respiratory syndrome coronavirus 2 (SARSCoV2) infection status. Here, we undertake a large scale study of audio-based deep learning classifiers, as part of the UK governments pandemic response. We collect and analyse a dataset of audio recordings from 67,842 individuals with linked metadata, including reverse transcription polymerase chain reaction (PCR) test outcomes, of whom 23,514 tested positive for SARS CoV 2. Subjects were recruited via the UK governments National Health Service Test-and-Trace programme and the REal-time Assessment of Community Transmission (REACT) randomised surveillance survey. In an unadjusted analysis of our dataset AI classifiers predict SARS-CoV-2 infection status with high accuracy (Receiver Operating Characteristic Area Under the Curve (ROCAUC) 0.846 [0.838, 0.854]) consistent with the findings of previous studies. However, after matching on measured confounders, such as age, gender, and self reported symptoms, our classifiers performance is much weaker (ROC-AUC 0.619 [0.594, 0.644]). Upon quantifying the utility of audio based classifiers in practical settings, we find them to be outperformed by simple predictive scores based on user reported symptoms.

==> extra_text/bits_of_possibly_useful_text.tex <==

($\predlab \perp \ylab \mid \zlab$). 

is likely to have a  which have the potential toFinally, relatively strong non-causal Covid associations driven by enrolment, classifiers are able to explain


    \begin{enumerate}
        \item 
        \item The classifier may learn self-reported symptoms at training stage, while neglecting latent non-self-identifiable symptoms. 
        \item While some self-reported symptoms are causally related to Covid, others may not be (e.g.\ a standard cough), and symptoms-based enrolment bias could lead the classifier to learn self-identifiable symptoms that are not causally related to Covid. 
    \end{enumerate}


A concern when training a classifier to predict \gls{covid} status from acoustic recordings is that its performance may be mediated by self-reported symptoms or other acoustically identifiable confounders (e.g.\ age, sex or ethnicity) that exhibit non-causal association with \gls{covid} due to biased study enrolment. This is illustrated in Figure~\ref{fig:causal_model}(a)(i) and (b)(i) where the association between classifier prediction and \gls{covid} status is mediated by symptoms ($\predlab \perp \ylab \mid \zlab$). 


General structure of our discussion of preferred acoustic target
\begin{enumerate}
    \item It seems universally desirable that the targeted acoustic signature should be caused by Covid. However, there are many ways in which the signature might relate to symptoms observed in \gls{covidneg}, e.g.\ the target could be
    \begin{enumerate}
        \item qualitatively Covid-specific (e.g.\ a continuous cough seen only in a small minority of \gls{covidneg})
        \item a quantitative change in symptoms seen in \gls{covidneg} (e.g.\ a louder cough)
    \end{enumerate}
    \item Some self-identifiable symptoms are causally linked to Covid (e.g.\ new continuous cough). Other self-identifiable symptoms may not show strong causal association with Covid  (e.g.\ a standard cough). How does our acoustic target relate to self-identifiable symptoms? 
    \begin{enumerate}
        \item A targeted acoustic signature that detects non-self-identifiable symptoms is of more practical benefit than one that detects self-identifiable symptoms because:
        \begin{enumerate}
            \item It is easier and more accurate to measure Covid-caused self-identifiable symptoms directly using a questionnaire than is to measure them indirectly via audio.
            \item Downstream, one can combine a latent-audio-symptom classifier with self-reported symptoms (causallly related to Covid) to increase performance
            \item As we see below, self-identifiable symptoms can affect enrolment, and therefore may be strongly non-causally associated with Covid in enrolled subpopulations 
        \end{enumerate}
    \end{enumerate}
    \item Non-randomised enrolment can induce non-causal association between Covid status and potentially audible individual-level characteristics such as 
    \begin{enumerate}
        \item Self-reported symptoms, whether caused by COVID-19 or not
        \item Confounders measured in metadata, e.g.\ age, sex, ethnicity
        \item Unmeasured confounders: accents specific to location, ...
    \end{enumerate}
    \item What are the consequences when we train our audio-based classifier in a population with non-causal associations between Covid and audible individual-level characteristics?
    \begin{enumerate}
        \item The classifier may learn to identify confounding variables that are not causally related to Covid, such as sex or age. Such an issue may go unnoticed if the test set is subject to the same enrolment biases as the training set.
        \item The classifier may learn self-reported symptoms at training stage, while neglecting latent non-self-identifiable symptoms. 
        \item While some self-reported symptoms are causally related to Covid, others may not be (e.g.\ a standard cough), and symptoms-based enrolment bias could lead the classifier to learn self-identifiable symptoms that are not causally related to Covid. 
    \end{enumerate}
    \item Matching is a tool to measure and control learning measured self-reported symptoms and other measured confounders 
    \begin{enumerate}
        \item Test-set matching of measured audible confounders (symptoms, age, sex) ensures that classifier performance is not mediated by the measured confounders (or any interactions amongst them). Continuous confounders, such as age, are discretized into bins
        \item Training-set matching of measured audible confounders encourages classifier to learn other audible characteristics, which may be either the targeted audio signature, or unmeasured confounders
        \item Matching can result in a reduced sample size, so it can be beneficial to design studies and recruit participants in such a way as to maximise the potential for matching on audible confounders in the enrolled cohort (give example)
    \end{enumerate}
    \item We attempt to quantify the effects of unmeasured confounders. One way of doing this is to assert that COVID-predictive variation that is seen amongst Covid negative participants is attributable to unmeasured confounders. This can be justified by defining our acoustic target accordingly. For example, we might define the acoustic target to be unusual in Covid negative participants.  
    \item The population in which we desire to detect Covid is often different to the population in which we wish to build our classifier.
    \begin{enumerate}
        \item At training stage, audio-based Covid classifiers benefit from a large sample size in both \gls{covidneg} and \gls{covidpos} groups (argument for balanced group sizes in ML?)
        \item However, the classifier may be intended for use in the general population, or in a particular clinical context
        \item We can change the loss function to reflect the population in which the classifier will be used (is this commonly done? [refs])
    \end{enumerate}
\end{enumerate}


Miscellaneous points:
\begin{enumerate}
    \item Is it possible to identify COVID signatures within a subset of the matched strata
\end{enumerate}


Covid classifier We compare the accuracy of self-reported symptoms status (any symptoms versus no symptoms) as a binary classifier of \gls{covid} status in these three subpopulations. The sensitivity, specificity, AUC, $R^2$ and \gls{mi} are shown below each of the tables in Figure~\ref{fig:bias_intro}. 

This \input{text_numbers/neg_prop_asym_us.txt}\unskip\% asymptomatic rate of \gls{covidneg} in our study is close to the estimated \input{text_numbers/react_estimated_neg_prop_asym.txt}\unskip\% asymptomatic rate among \gls{covidneg} individuals in the general population at the time of enrolment.\footnote{This \input{text_numbers/react_estimated_neg_prop_asym.txt}\unskip\% is a simple estimate based on the self-reported asymptomatic rate amongst \gls{covidneg} \gls{react} participants in our study; this could deviate from the true population asymptotic rate due to enrolment bias.} However, the \input{text_numbers/pos_prop_asym_us.txt}\unskip\% asymptomatic rate of \gls{covidpos} participants in our study is an order of magnitude smaller than the 35\% asymptomatic rate amongst \gls{covidpos} individuals in the general population, as estimated by large meta analyses \cite{oran_proportion_2021,sah_asymptomatic_2021}. 

These high-level statistics provide a useful introduction to the potentially misleading effects of enrolment bias. 
Figure~\ref{fig:bias_intro} shows the joint distribution of \gls{covid} status and symptoms status in subpopulations generated by: (a) randomised enrolment by taking a random sample from the general population; (b) biased enrolment in which \gls{covidpos} individuals are preferentially sampled based upon their symptoms status; and (c) matched enrolment, in which the number of \gls{covidpos} and \gls{covidpos} individuals are the same for each particular symptoms profile, here within symptomatic and asymptomatic strata. 

Note the strong predictive accuracy in our enrolled subpopulation (AUC = \input{text_numbers/auc_us.txt}\unskip), compared to the weak predictive accuracy in the general population (AUC = \input{text_numbers/auc_genpop.txt}\unskip). 

\footnote{For illustrative purposes we have assumed \gls{covid} prevalence of 2\% in the general population.}

Now consider an audio-based classifier that distinguishes accurately between symptomatic and asymptomatic individuals. This audio-based classifier will also predict \gls{covid} status accurately in our ascertained study, while performing poorly at predicting \gls{covid} status in the general population. 

Thinking more generally, the enrolment bias does not have to work through symptoms. It can work through any confounding variables that are predictive of Covid statusIf the audio-based classifier is unable to classify symptoms perfectly,  

but they are pretty clear: an audio-based classifier that is able to distinguish between those who are symptomatic or not will perform very well at predicting Covid in our ascertained study, but will have no useful predictive accuracy in the general population.

The causal mechanisms underlying this discrepancy are presented in Figure X in a Bayesian knowledge graph. reasons for this discrepancy are shown in Figure X. 

\todo{}{Additional Table(s)/Figure(s) of cohort characteristics? Let's finalise what else we want to show and how we want to present it.}

Pillar 1 tests refer to \textit{``all swab tests performed in \gls{phe} labs and \gls{nhs} hospitals for those with a clinical need, and health and care workers''}, and Pillar 2 comprises \textit{``swab testing for the wider population''} \cite{department_of_health_and_social_care_uk_covid-19_nodate}. Pillar 1+2 testing thus has more capacity than the randomised programs, but the protocol incurs ascertainment bias as those at elevated risk of being infected are tested, such as frontline workers, contacts traced to a \gls{covid} case, or the sub population presenting with \gls{covid} symptoms, such as loss of taste and smell \cite{department_of_health_and_social_care_uk_covid-19_nodate}.

The effect can be summarised as follows: \gls{covid} cases are much more likely to have symptoms than are controls, amongst those individuals ascertained for any given data set. This allows audio-based AI classifiers to pick up on symptoms and hence perform well on in-sample accuracy within these data sets, without possessing any generalisable out-of-sample utility over and above self-reported symptoms. 

In our study we control for symptoms-based recruitment. We do this via the standard epidemiological method of matching, whereby we balance cases and controls in each of several key strata, carefully constructed with respect to gender, age, and symptoms. In the matched data set, by construction, we remove any confounding association between acoustics and COVID status as mediated by gender, age or symptoms. 




%  First, self-reported symptoms can be used to diagnose \gls{covid} with reasonably high accuracy, particularly in study subpopulations, such as ours, that are enrolled based on symptoms. Second, 
% Proposition 1: Study enrolment often leads to strong non-causal associations between \gls{covid} status and audible characteristics of individuals, such as self-reported symptoms, age, sex and ethnicity.

% \textbf{Proposition 1:} Self-reported symptoms can be used to diagnose \gls{covid} with reasonably high accuracy, particularly in study subpopulations, such as ours, that are enrolled based on symptoms.
% \textbf{Proposition 2:} diagnosing \gls{covid} indirectly via audio-based recognition of self-reported symptoms is not clinically useful, as it is easier and more effective to measure those self-reported symptoms directly via a questionnaire; importantly, this is in contrast to the potentially substantial benefit of learning a latent \gls{covid} audio signature that cannot be readily identified and reported by humans themselves. 


% This is not to suggest that Covid-caused self-identifiable symptoms are not useful for predicting Covid, it is simply to say that  


% \begin{enumerate}
%     \item Self-reported symptoms, whether caused by COVID-19 or not
%     \item Confounders measured in metadata, e.g.\ age, sex, ethnicity
%     \item Unmeasured confounders: accents specific to location, ...
% \end{enumerate}




% Brief scene-setting including
% \begin{enumerate}
%     \item Overview of \gls{covid} pandemic - number deaths, hit to economy
%     \item Why it is important to diagnose Covid early and effectively. (self-isolation, tracking population spread for logistical preparation, vaccination/boosting, and non-pharmaceutical intervention, early administration of pharmaceuticals in clinical settings,...)
%     \item \gls{pcr} and LFD tests, sensitivity and specificity, ...
%     \item Medical imaging (CT, X-ray, ultrasound), ...  \cite{born_role_2021}
%     \item Audio-based Covid diagnosis -- what are the costs, (dis)advantages, benefits relative to other approaches?
% \end{enumerate}


% A key balance to be struck is the trade-off between extent of population quarantined and protection of the economy. 

% Over the course of the \gls{covid} pandemic two main tests for the disease have been used: The \gls{pcr} test and the \gls{lft}. \gls{pcr} tests represent the gold standard but are costly, requiring expensive machinery, which limits their availability. \gls{lft}s are considerably cheaper and can be conducted by members of the public, making them widely available. However, their performance at detecting the disease is less good \cite{Moysen90}  with some reporting sensitivity scores as low as 58 \% when the test is conducted by a member of the public \cite{Deekse2022}.



% We have identified 19 \gls{covid} respiratory audio datasets in the published literature. We note here some general limitations which affect the majority of these collected datasets. Namely all represent relatively few \gls{covidpos} participants, with numbers ranging from 7 to 2660. Models trained and evaluated on so few cases are unlikely to generalise well. The majority of datasets did not verify the participants' reported \gls{covid} status, and many did not specify a preference between \gls{pcr} and the less reliable \gls{lft}. This lack of label verification puts into question the validity of the dataset's labels and extends to a problem of lack of control over the delay between testing and recording audio. A maximum time delay between the dates of the testing and recording should be specified, a step not possible if the date of the test is unknown. \todo{harry}{finish off limitations. Lack of metadata, environmental corruption, participant disjoint sets. We need to contextualise this against the discussion in Han. Also we should try to be constructive rather than negative about previous work.}



% and lack of applicability of prediction models. %\cite{wolff_probast_2019} or, more specifically 
% For example, Roberts \textit{et al.} performed a systematic review of 62 imaging-based studies (chest radiographs or \gls{ct} scans) and adjudged none of those models to be of potential clinical use due to methodological flaws and/or underlying biases \cite{roberts_common_2021-1}. 
% \begin{itemize}
%     \item Overfitting of data (e.g.\ failure to perform cross validation via a training/validation/test data split)
%     \item A small sample size of patients with COVID-19, leading to imbalanced data sets
%     \item Participant enrolment bias
%     \begin{itemize}
%         \item Study populations not being representative of the wider targeted population
%         \item Systematic differences in characteristics between the COVID-19 cohort and the control groups
%         \item Were inclusion/exclusion of participants appropriate and reproducible
%     \end{itemize}
%     \item Lack of appropriate evaluation of the performance metrics (for example, no discussion of calibration/discrimination)
%     \item Unclear or inaccurate \gls{covid} status 
% \end{itemize}




% In our initial analysis, we observed strong classifier performance as previously reported in other studies. However, upon controlling for confounding in our dataset we observed strongly reduced \gls{covid} diagnostic performance, not much better than a random guess. We hypothesise this confounding effect to be a property of \gls{covid} audio datasets more generally.




% \subsection*{Our contribution}


% \begin{enumerate}
%     \item Here we report the findings of the largest study to date, evaluating the performance of two complementary AI based audio classifiers, with \input{text_numbers/tot_us.txt} individuals with linked \gls{pcr} test outcomes, of whom \input{text_numbers/pos_tot_us.txt} tested positive for \gls{covid}, undertaken in partnership with the UK Health Security Agency (UKHSA).\todo{}{Introduction to the Turing-RSS Health Data Lab and UKHSA partnership.}
%     \item Our main research question is: "Can audio recordings serve as a tool for improving diagnosis of \gls{covid}?" and in particular whether audio-based classifiers offer improved diagnostic accuracy beyond that achieved based on self-reported symptoms? 
%     \item In our basic analyses, we observe strong classifier performance as previously reported in other studies.
%     \item However, there are strong participant enrolment effects in our study and, upon controlling for for this, we observe strongly reduced \gls{covid} diagnostic performance, not much better than a random guess. We hypothesise this study-enrolment effect to be a property of \gls{covid} audio datasets more generally. 
%     \item We outline existing statistical approaches to reducing and controlling for enrolment bias, discussing how they can best be applied in the context of highly parameterised machine learning models.
%     % These measures can be implemented both the design and analysis stages. 
%     \item We feel that our message is timely and important from the perspective of preventing the potential of  misinterpreting audio-based classifier outputs. There is an additional important general point to be made about confounding in AI-based epidemiology -- a situation in which biases are often hard to spot and difficult to control for.
%     \item Our data set will be made publicly available.\footnote{The UKHSA are committed to making the study data openly available with an accompanying description to be submitted to Nature Scientific Data.}
%     \item In our study we used a pre-specified analysis plan to promote replicability of conclusions.
% \end{enumerate}



% We at the \href{https://www.turing.ac.uk/research/research-projects/turing-rss-health-data-lab}{The Turing-RSS Health Data Lab}, in partnership with the \href{https://www.gov.uk/government/organisations/uk-health-security-agency}{UK Health Security Agency (UKHSA)}, set out 



% ``Can audio recordings serve as a tool for improving diagnosis of \gls{covid}?'' and in particular whether audio-based classifiers can be used to diagnose accurately beyond that achieved based on self-reported symptoms. 

% % who have no medical training, and who have access only to common diagnostic tools such as a thermometer). 

% % Third, if our audio-based classifier is able to diagnose Covid through non-self-identifiable symptoms, then it can be can be used post hoc to augment predictions based on self-reported symptoms.
% % This could be qualitative rarity (e.g.\ a new, continuous cough not observed in Covid negatives) or quantitative rarity (e.g.\ Covid positives have a louder version of the cough seen commonly in Covid negatives \todo{all}{Can we find a better example of qualitative rarity}). 

% In other cases, methodological flaws are identified, e.g.\ the overfitting of small datasets with complex models, or allowing the same individuals to appear in both training and test sets. 

% In particular, if an individual's enrolment in a study is determined by their characteristics (as opposed to randomised selection from population), then enrolment can induce additional non-causal association between \gls{covid} status and those characteristics. This is especially problematic when these characteristics are predictable from acoustic recording, such as self-identifiable symptoms (whether caused by \gls{covid} or not), age, gender or ethnicity. 
% , i.e.\ stratified according to whether participants are \gls{covidpos} or \gls{covidneg}. 
% There is a striking difference in symptoms profiles between the \gls{covidpos} and \gls{covidneg} subgroups, with \input{text_numbers/neg_prop_asym_us.txt}\unskip\% (\input{text_numbers/neg_asym_us.txt}\unskip\ of \input{text_numbers/neg_tot_us.txt}\unskip) of \gls{covidneg} individuals asymptomatic, in contrast to only \input{text_numbers/pos_prop_asym_us.txt}\unskip\% (\input{text_numbers/pos_asym_us.txt}\unskip\ of \input{text_numbers/pos_tot_us.txt}\unskip) of \gls{covidpos} individuals. 


% The node labelled ``Covid acoustic signature'' is the hypothesised latent audio indication of interest; note that it is distinct from ``self-reported symptoms'' which has its own node. 

% , and the causal association is represented in Figure~\ref{fig:causal_model}(b)(i) by a narrow line, labelled $R^2$=\input{text_numbers/r2_genpop.txt}\unskip\ with reference to Figure~\ref{fig:bias_intro}(b).


% by preventing the performance of several analyses followed by presentation of the most favourable result\cite{kahan_how_2020}.
% (commonly referred to as ‘p-hacking’) multiple-testing burden incurred through multiple iterations of different analyses.
% ions of repeated iterations of model fitting and refinement on variously oriented data (also known as p-hacking or mining for spurious relationships). 

% The first step of the plan was to analyse the collected dataset and identify confounding factors. Then, based on this analysis, construct train and test splits to mitigate this bias. 

% Having observed low predictive accuracy in Matched and Longitudinal Matched test sets considering all matched strata collectively, 

% , or whether we might observe systematically better performance in certain matched strata. 




% In terms of methodological alternatives to matching in this context,  There are alternative approaches as well, for example the literature on fairness in AI, whereby classifiers are trained to perform equitably with respect to certain protected characteristics.to training means for ensuring classifiers  performed matching  measured confounders) using matching. by matching

%  Methodologically, 


%  to allay these concerns, and move forwards to a definitive characterisation of whether there is added utility available through \gls{abcd}.


% into 
% effectiveness of  have conducted the in the largest study of it is kind to date, we identify the important role of symptoms-based recruitment bias in \gls{abcd}. , demonstrating how such bias artificially inflates estimates of prediction accuracy. Our study's dataset harbours a sizeable component of Covid-predictive variation that is attributable to self-identifiable symptoms-based recruitment. , as opposed to a useful Covid-predictive acoustic signature.

% \begin{enumerate}
%     % \item Limitations of our study
%     % \begin{enumerate}
%     %     \item 
%     % \end{enumerate}
%     \item Broader implications for audio–based classification of Covid and other outcomes in AI/ML
%     \begin{enumerate}
%         \item How often is true out-of-sample classification performance exaggerated due to confounding? In Covid audio-based prediction? More generally in audio-based prediction?
%         \item Difficulties in establishing causality---unmeasured confounders in training studies may lead to low generalisability.
%     \end{enumerate}

%     \item Future directions for addressing enrolment bias in AI
%     \begin{enumerate}
%         \item Development, and more widespread use, of methods for adjusting for bias when training classifiers. There is already much work on fairness in AI, whereby classifiers are trained to perform equitably with respect to certain protected characteristics. 
%         % (How this relates to fairness in AI,  How this relates to causal inference)
%     \end{enumerate}

% \end{enumerate}

% We believe that this will constitute compelling evidence that audio-based prediction of COVID in ascertained cohorts is mostly, if not entirely, mediated by symptoms and, as such, offers no clinical utility beyond user-completed health questionnaires.


% We can summarise our novel insights into the problem of recruitment bias as follows. 

% The essential problematic elements of selection bias in \gls{abcd} may be summarised as follows: 
%     % \item We believe that symptoms-based enrolment poses a major obstacle to the creation of useful classifiers in \gls{abcd} generally. 
% \begin{enumerate}
%     \item Covid is causally related to particular self-identifiable symptoms, such as a new continuous cough. This has allowed such symptoms to be used as a basis for population intervention to control disease spread, all via self-diagnosis and without recourse to audio recording. It is therefore desirable to develop audio-based classifiers that can augment and complement the information provided by self-identifiable Covid-specific symptoms, i.e.\ to learn clinically valuable \textit{latent} acoustic signatures caused by Covid.  
%     \item Problematically, enrolment based on symptoms has the potential not only to artificially inflate the association between Covid and its particular symptoms, but also to introduce association between Covid and symptoms that are not Covid-specific. Furthermore, enrolment based upon other characteristics, such as gender and age, may additionally introduce non-causal Covid-to-gender or Covid-to-age associations in the enrolled subpopulation, \textit{possibly interacting with symptoms}.
%     \item Under such recruitment bias, classifiers trained to predict Covid in enrolled subpopulations may learn to predict \textit{self-identifiable} Covid-specific symptoms, thereby providing no additional utility beyond a classifier trained directly on those self-diagnosed symptoms. Worse, the classifier may learn to predict age/gender/non-Covid-specific symptoms as proxies for Covid in the enrolled subpopulation, in which case the its performance will not generalise to subpopulations unaffected by the same recruitment bias. 
%     % Because non-causal Covid-to-(symptoms/age/gender/...) associations the entire enrolled subpopulation, ``audio-based symptoms/age/gender predictors'' can also achieve high performance in held-out test sets.
%     % \item 
%     % provided by the causal relationship between Covid and its particular symptoms. 
%     % When applied in realistic settings, such as in the general population, ``audio-based symptoms/age/gender predictors'' may provide little additional utility beyond a non-audio classifier based only upon self-identifiable symptoms trained in that setting.
%     % \item  Matching is one methodological means of assessing whether a classifiers' predictive accuracy exceeds the accuracy offered by symptoms alone, though there remains the challenge posed by unmeasured confounders. In the end, utility may be best assessed by carefully quantifying the utility of audio-based classifiers by piloting them in real-world settings,  and comparing their utility to that of non-audio classifiers, e.g.\ based only on self-identifiable symptoms, in the same context.
% \end{enumerate}

% There is well known to be a true causal association linking Covid and some self-identifiable symptoms in the general population (e.g.\ \gls{roc}=75\% in Figure~\ref{fig:bias_intro}(b)) which has provided a useful interventional tool to control disease spread (without recourse to audio recording). However, when study enrolment is dependent upon participant characteristics, such as symptoms/age/gender, there is the potential for strong non-causal relationships to be induced between these characteristics and Covid status in the in enrolled subpopulation. Covid status and interactions of can be introduced  

% The undesirable effects of symptoms-based recruitment are conceptually complicated, because of the  The fundamental issue is that enrolment can artificially induce strong non-causal Covid-to-symptoms association in the enrolled subpopulation (e.g.\ \gls{roc}=87\% in Figure~\ref{fig:bias_intro}(a)); this has the potential both to artificially inflate the causal association in (A), and also to introduce association between Covid and symptoms that are not causally related to it. Enrolment based upon other characteristics, such as gender and age, may additionally introduce non-causal Covid-to-gender or Covid-to-age associations in the enrolled subpopulation, possibly interacting with symptoms.



% The first involves constructing a space where it is hypothesised the \gls{covidpos} signal is projected to the null space. On the assumption \gls{covidpos} signal exists in an orthogonal space to the rest of human respiratory sound features we project the dataset onto the principal components of just the \gls{covidneg} individuals. In this space variance is maximised for \gls{covidneg} but the variance in \gls{covidpos} is not. Classifiers which perform well in this constructed space are hypothesised to be leveraging a signal which 

% Examples of unaccounted for bias include, participant's symptoms which have not been reported and environmental corruption, such as correlations between background noise and \gls{covid} status, for example hospital noise. 

% Put the logistic regression into the analysis above "Characterising predictive variation in Naive test set"
% \paragraph{Logistic Regression on symptoms} \textcolor{red}{How well does a categorical logistic regression model perform at \gls{covid} classification}

%Our approach is enabled by the rarity property of the targeted acoustic signature, i.e.\ that it is rarely observed in \gls{covidneg} individuals. If the audio variation underlying the residual ROC-AUC$\approx$0.6 is common in \gls{covidneg} individuals, then we attribute it to unmatched/unmeasured confounders. 



% In the Matched test set 3 of 19 strata show statistically significant association between predictions and COVID status; in the Longitudinal Matched test set a greater number, 10 of 19 strata, are significant reflecting the greater sample size (in both cases controlling \gls{fdr} at 5\%). Stratum-specific predictions and results are detailed in Figure~\ref{fig:stratified_roc-auc}. this


% The sample size is higher in the This is supportive of a weak predictive across multiple It is informative that we observe the majority of strata significant in the Longitudinal Matched test set


% Taking the null that the trained model's predicted probability for \gls{covidpos} is no higher than for \gls{covidneg} test recordings in a particular strata, we perform the nonparametric unpaired Mann-Whitney-Wilcoxon test. After accounting for \gls{fdr} using the Benjamini-Hochberg procedure, we see three significant rejections of the null. 

% These results are detailed in Figure~\ref{fig:stratified}. Three different strata reject the null in both the matched training and standard training set up. While these strata are similar, all being female and similar age ranges, they do not match perfectly. These associations may be suggestive (among other things) of (i) some useful predictive ability in these subgroups and/or (ii) unmeasured/uncontrolled confounders driving an association in these strata particularly. \todo{harry + george}{repeat for long matched test set}

% , both of which are only minor improvements over a ``random-guess'' ROC-AUC of 0.5. In the Longitudinal Matched test set,  


% When we train the \gls{ssast} classifier on the Matched training set, we observe a small improvement in performance on the Matched test set ROC-AUC=0.635$\pm$XXX, consistent with the model learning alternative associated pathways to COVID, either via the targeted acoustic signature or via unmatched/unmeasured confounders (Figure~\ref{fig:causal_model}(c)(iii)). 

% Here the models' classification performances are reported for all four respiratory audio modalities (sentence, three cough, cough and ha sound). For each modality the nine experiments detailed in the pre-specified analysis plan are shown. For each evaluation \gls{uar}, \gls{roc} and \gls{pr} metrics are reported. The two pre-specified models, openSMILE-\gls{svm} and \gls{ssast} were evaluated on these tasks. The general trend, which has been highlighted by the emboldened scores in Table~\ref{tab:main-results}, is that \gls{ssast} consistently outperforms the baseline, with the sentence and ha sound modalities proving to be the top and bottom performing signals respectively.

% The most important result for this study is that without ascertainment bias adjustment, we observe \gls{COVID} predictive accuracy with a ROC-AUC of 0.846 $\pm$ 0.006 (consistent with existing studies)\footnote{SSAST achieved \gls{roc} scores of 0.846, 0.809, 0.790 and 0.750 on sentence, three cough, cough and ha sound respectively in an unadjusted setting.}. However, when we control for ascertainment bias through matching, we find predictive accuracy with ROC-AUC of 0.619 $\pm$ 0.026\footnote{SSAST achieved \gls{roc} scores of 0.619, 0.577, 0.561 and 0.581 on sentence, three cough, cough and ha sound respectively in the matched test set.}. This presents a minor improvement over a random guess (ROC-AUC 0.5), which in itself may be due to further unaccounted confounding. \todo{harry}{add confidence intervals} \todo{harry}{is it significantly better than random?}

% In an attempt to boost performance through training our models in a confounder adjusted setting, we train the models on the matched training set. Here we see a performance gain on the matched test set however, a slight drop in performance on the three other test sets. Interestingly we see no performance decrease between the standard test set and the longitudinal test set. It is also important to note that the performance gap between \gls{ssast} and openSMILE-\gls{svm} is greatly reduced for the matched test sets compared to the standard, longitudinal and naive settings.


% The results are qualitatively similar for the other scenarios having 10\% and 30\% symptomatic \gls{covidneg} individuals in Figure~\ref{fig:audio_vs_symptoms_genpop}(a) and (c) respectively. 


% Focusing on the general population with 20\% of \gls{covidneg} symptomatic (Figure~\ref{fig:audio_vs_symptoms_genpop}(b)) we see a number of noteworthy results. the main conclusion is that the Symptoms+Audio \gls{rf} classifier offers a significant (p=3.6E-9) but small improvement in accuracy compared to the Symptoms \gls{rf} classifier, and


% Especially in light of this potential bias, it is noteworthy that the additional predictive accuracy conferred by 


% .  but significant improvement over a  symptoms small but significant only marginal
% As indicated by the non-overlapping CIs, the ROC−AUC significantly higher for the Symptoms+Audio \gls{rf} vs the 



% \subsubsection*{Measuring utility of classifiers}


% supplement generic measures of predictive accuracy such as ROC-AUC, sensitivity and specificity, 
% we can tailor a utility function . This involves specifying the characteristics of the population in which testing is to be performed (particularly the prevalence), and the utility of true (and false) positives and negatives. 


% The first experiments, labelled . Next a  From this Standard test set, a `Matched' test set was This was carefully constructed with respect to gender, age, and symptoms. In the Matched data set, by construction, we removed any confounding association between acoustics and COVID status as mediated by gender, age or symptoms. To test for covariate shift with time, a `Longitudinal' test set was constructed so that any participant joining the study after 29\textsuperscript{th} November 2021 would only feature in the Longitudinal test set. An additional `Matched Longitudinal' test, employing the same methods for the Matched test set but on the Longitudinal test set was created.




% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{figs/stratified_analysis_input_file_ss_predics.jpg} \\
%     \includegraphics[width=\textwidth]{figs/stratified_analysis_input_file_ss_predics_matched_train_2.jpg} 
%     \caption{Strata in the Matched test set which significantly rejected the null (FDR accounted for through the Benjamini–Hochberg procedure) that \gls{covid} +ve individuals are not distinguishable from their respiratory sounds compared to \gls{covid} -ve individuals in the Matched test set. The Matched training set refers to when the model is trained on the Matched training set and then evaluated on the Matched test set. The full training set refers to when the model is trained on the standard training set and evaluated on the Matched test set. The model used in these experiments was \gls{ssast} and here we see the results for the sentence modality.}
%     \label{fig:stratified}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{figs/stratum_plots.pdf}
%     % \caption{Strata in the Matched test set which significantly rejected the null (FDR accounted for through the Benjamini–Hochberg procedure) that \gls{covid} +ve individuals are not distinguishable from their respiratory sounds compared to \gls{covid} -ve individuals in the Matched test set. The Matched training set refers to when the model is trained on the Matched training set and then evaluated on the Matched test set. The full training set refers to when the model is trained on the standard training set and evaluated on the Matched test set. The model used in these experiments was \gls{ssast} and here we see the results for the sentence modality.}
%     \caption{Exploration within strata.}
%     \label{fig:stratified}
% \end{figure}





% The essential elements of our concerns about selection bias in \gls{abcd} may be summarised as follows: 
%     % \item We believe that symptoms-based enrolment poses a major obstacle to the creation of useful classifiers in \gls{abcd} generally. 
% \begin{enumerate}
%     \item[] (A) There is a causal association linking Covid and self-identifiable symptoms in the general population (e.g.\ \gls{roc}=75\% in Figure~\ref{fig:bias_intro}(b)) which has provided a useful interventional tool to control disease spread (without recourse to audio recording).
%     \item[] (B) Symptoms-based enrolment can artificially induce strong non-causal Covid-to-symptoms association in the enrolled subpopulation (e.g.\ \gls{roc}=87\% in Figure~\ref{fig:bias_intro}(a)); this has the potential both to artificially inflate the causal association in (A), and also to introduce association between Covid and symptoms that are not causally related to it. Enrolment based upon other characteristics, such as gender and age, may additionally introduce non-causal Covid-to-gender or Covid-to-age associations in the enrolled subpopulation, possibly interacting with symptoms.
%     \item[] (C) Because of (B), classifiers trained to predict Covid in enrolled subpopulations are often just ``audio-based symptoms/age/gender predictors'', i.e.\ they learn to predict self-identifiable symptoms/age/gender as proxies for Covid in the enrolled subpopulation, instead of learning potentially valuable latent acoustic signatures caused by Covid (should such signatures exist).
%     \item[] (D) Because (B) can induce strong non-causal Covid-to-(symptoms/age/gender/...) association across thtire enrolled subpopulation, ``audio-based symptoms/age/gender predictors'' can also achieve high performance in held-out test sets.
%     \item[] (E) When applied in realistic settings, such as in the general population,  ``audio-based symptoms/age/gender predictors'' may provide little additional utility beyond a non-audio classifier based only upon self-identifiable symptoms trained in that setting.
%     \item[] (F) It is desirable to develop audio-based classifiers that can augment and complement the information provided by self-identifiable symptoms. Matching is one methodological means of assessing whether a classifiers' predictive accuracy exceeds the accuracy offered by symptoms alone, though there remains the challenge posed by unmeasured confounders. In the end, utility may be best assessed by carefully quantifying the utility of audio-based classifiers by piloting them in real-world settings,  and comparing their utility to that of non-audio classifiers, e.g.\ based only on self-identifiable symptoms, in the same context.
% \end{enumerate}



% Algorithm PCA 2
% \begin{enumerate}
%     \item For \# PCs $k = 1:K$
%     \begin{enumerate}
%         \item Project \gls{covidpos} and \gls{covidneg} openSMILE features onto the first $k$ principal components of the \gls{covidneg} cases
%         \item Train and evaluate SVM in k-dimensional PCA-reduced Matched test set
%     \end{enumerate}
%     % \item Train an evaluate an \gls{svm} classifier on progressively more principal components. The fewer components the weaker the model.
%     % \item Cases which the weak model is able to classify correctly are removed from the Matched test set to create a curated Matched test set.
% \end{enumerate}

% Our general conclusion from Figure~\ref{fig:audio_vs_symptoms_genpop}(d)-(f) the Symptoms+Audio classifier compared to the Symptoms classifier also increases 



% (e.g.\ it may depend on the joint distribution of symptoms and \gls{covid}, as illustrated in Figure~\ref{fig:bias_intro}(a) and \ref{fig:bias_intro}(b), which will vary according to seasonal variation in the proportion of symptomatic \gls{covid} negatives). 




% In each case, the estimated \gls{roc} is greater in the Symptoms \gls{rf} classifier than in the Audio \gls{rf} classifier; e.g.\ in   In the 


% ROC−AUC: 0.780 (0.766−0.794) − Symptoms+Audio

% We then quantify sensitivity, specificity and utility in this ``general population'' test set.
% designed to contain the actual Covid-to-symptoms association observed in the general population during the pandemic. 

% The purely age/gender/symptoms-based classifier outperforms the audio-based classifier in terms of ROC-AUC (0.694 (0.663−0.726) vs 0.677 (0.644−0.710)). Given these sensitivity/specificity relationships, we can go on to calculate and maximise the expected utility, as defined at \eqref{eq:expected_utility}, for any particular value of the general population Covid prevalence $\pi$ and utility function $\B{u}$. 

% \paragraph{Characterising predictive variation in Naive test set.} We examine the hypothesis that the high predictive accuracy of \gls{roc}=0.846 is mediated by self-reported symptoms (which exhibit non-causal enrolment-induced association with \gls{covid}). We train a classifier that is a known symptoms detector (but not a \gls{\gls{covid}} detector) by filtering the training data to include only \gls{covidneg} individuals, and training an audio-based classifier on binary self-reported symptoms (asymptomatic vs symptomatic). When evaluated at \gls{covid} detection these binary symptoms classifiers achieve classification scores of 0.69 and 0.73 \gls{roc} for the openSMILE-\gls{svm} and \gls{ssast} models respectively on the naive test set. 


==> extra_text/sn_example_text.tex <==
% COVID-19 detection from Audio
%%==================================%%
%% sample for unstructured abstract %%
%%==================================%%

%%================================%%
%% Sample for structured abstract %%
%%================================%%

% \abstract{\textbf{Purpose:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.
% 
% \textbf{Methods:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.
% 
% \textbf{Results:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.
% 
% \textbf{Conclusion:} The abstract serves both as a general introduction to the topic and as a brief, non-technical summary of the main results and their implications. The abstract must not include subheadings (unless expressly permitted in the journal's Instructions to Authors), equations or citations. As a guide the abstract should not exceed 200 words. Most journals do not set a hard limit however authors are advised to check the author instructions for the journal they are submitting to.}


%%\pacs[JEL Classification]{D8, H51}

%%\pacs[MSC Classification]{35A01, 65L10, 65L12, 65L20, 65L70}



%%=============================================================%%
%% Prefix	-> \pfx{Dr}
%% GivenName	-> \fnm{Joergen W.}
%% Particle	-> \spfx{van der} -> surname prefix
%% FamilyName	-> \sur{Ploeg}
%% Suffix	-> \sfx{IV}
%% NatureName	-> \tanm{Poet Laureate} -> Title after name
%% Degrees	-> \dgr{MSc, PhD}
%% \author*[1,2]{\pfx{Dr} \fnm{Joergen W.} \spfx{van der} \sur{Ploeg} \sfx{IV} \tanm{Poet Laureate} 
%%                 \dgr{MSc, PhD}}\email{iauthor@gmail.com}
%%=============================================================%%

% \author*[1,2]{\fnm{First} \sur{Author}}\email{iauthor@gmail.com}

% \author[2,3]{\fnm{Second} \sur{Author}}\email{iiauthor@gmail.com}
% \equalcont{These authors contributed equally to this work.}

% \author[1,2]{\fnm{Third} \sur{Author}}\email{iiiauthor@gmail.com}
% \equalcont{These authors contributed equally to this work.}

% \affil*[1]{\orgdiv{Department}, \orgname{Organization}, \orgaddress{\street{Street}, \city{City}, \postcode{100190}, \state{State}, \country{Country}}}

% \affil[2]{\orgdiv{Department}, \orgname{Organization}, \orgaddress{\street{Street}, \city{City}, \postcode{10587}, \state{State}, \country{Country}}}

% \affil[3]{\orgdiv{Department}, \orgname{Organization}, \orgaddress{\street{Street}, \city{City}, \postcode{610101}, \state{State}, \country{Country}}}


% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

% \section{This is an example for first level head---section head}\label{sec3}

% \subsection{This is an example for second level head---subsection head}\label{subsec2}

% \subsubsection{This is an example for third level head---subsubsection head}\label{subsubsec2}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. 

% \section{Equations}\label{sec4}

% Equations in \LaTeX\ can either be inline or on-a-line by itself (``display equations''). For
% inline equations use the \verb+$...$+ commands. E.g.: The equation
% $H\psi = E \psi$ is written via the command \verb+$H \psi = E \psi$+.

% For display equations (with auto generated equation numbers)
% one can use the equation or align environments:
% \begin{equation}
% \|\tilde{X}(k)\|^2 \leq\frac{\sum\limits_{i=1}^{p}\left\|\tilde{Y}_i(k)\right\|^2+\sum\limits_{j=1}^{q}\left\|\tilde{Z}_j(k)\right\|^2 }{p+q}.\label{eq1}
% \end{equation}
% where,
% \begin{align}
% D_\mu &=  \partial_\mu - ig \frac{\lambda^a}{2} A^a_\mu \nonumber \\
% F^a_{\mu\nu} &= \partial_\mu A^a_\nu - \partial_\nu A^a_\mu + g f^{abc} A^b_\mu A^a_\nu \label{eq2}
% \end{align}
% Notice the use of \verb+\nonumber+ in the align environment at the end
% of each line, except the last, so as not to produce equation numbers on
% lines where no equation numbers are required. The \verb+\label{}+ command
% should only be used at the last line of an align environment where
% \verb+\nonumber+ is not used.
% \begin{equation}
% Y_\infty = \left( \frac{m}{\textrm{GeV}} \right)^{-3}
%     \left[ 1 + \frac{3 \ln(m/\textrm{GeV})}{15}
%     + \frac{\ln(c_2/5)}{15} \right]
% \end{equation}
% The class file also supports the use of \verb+\mathbb{}+, \verb+\mathscr{}+ and
% \verb+\mathcal{}+ commands. As such \verb+\mathbb{R}+, \verb+\mathscr{R}+
% and \verb+\mathcal{R}+ produces $\mathbb{R}$, $\mathscr{R}$ and $\mathcal{R}$
% respectively (refer Subsubsection~\ref{subsubsec2}).

% \section{Tables}\label{sec5}

% Tables can be inserted via the normal table and tabular environment. To put
% footnotes inside tables you should use \verb+\footnotetext[]{...}+ tag.
% The footnote appears just below the table itself (refer Tables~\ref{tab1} and \ref{tab2}). 
% For the corresponding footnotemark use \verb+\footnotemark[...]+

% \begin{table}[h]
% \begin{center}
% \begin{minipage}{174pt}
% \caption{Caption text}\label{tab1}%
% \begin{tabular}{@{}llll@{}}
% \toprule
% Column 1 & Column 2  & Column 3 & Column 4\\
% \midrule
% row 1    & data 1   & data 2  & data 3  \\
% row 2    & data 4   & data 5\footnotemark[1]  & data 6  \\
% row 3    & data 7   & data 8  & data 9\footnotemark[2]  \\
% \botrule
% \end{tabular}
% \footnotetext{Source: This is an example of table footnote. This is an example of table footnote.}
% \footnotetext[1]{Example for a first table footnote. This is an example of table footnote.}
% \footnotetext[2]{Example for a second table footnote. This is an example of table footnote.}
% \end{minipage}
% \end{center}
% \end{table}

% \noindent
% The input format for the above table is as follows:

% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%
% \bigskip
% \begin{verbatim}
% \begin{table}[<placement-specifier>]
% \begin{center}
% \begin{minipage}{<preferred-table-width>}
% \caption{<table-caption>}\label{<table-label>}%
% \begin{tabular}{@{}llll@{}}
% \toprule
% Column 1 & Column 2 & Column 3 & Column 4\\
% \midrule
% row 1 & data 1 & data 2	 & data 3 \\
% row 2 & data 4 & data 5\footnotemark[1] & data 6 \\
% row 3 & data 7 & data 8	 & data 9\footnotemark[2]\\
% \botrule
% \end{tabular}
% \footnotetext{Source: This is an example of table footnote. 
% This is an example of table footnote.}
% \footnotetext[1]{Example for a first table footnote.
% This is an example of table footnote.}
% \footnotetext[2]{Example for a second table footnote. 
% This is an example of table footnote.}
% \end{minipage}
% \end{center}
% \end{table}
% \end{verbatim}
% \bigskip
% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%

% \begin{table}[h]
% \begin{center}
% \begin{minipage}{\textwidth}
% \caption{Example of a lengthy table which is set to full textwidth}\label{tab2}
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
% \toprule%
% & \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]} & \multicolumn{3}{@{}c@{}}{Element 2\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
% Project & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
% \midrule
% Element 3  & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$\\
% Element 4  & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$\\
% \botrule
% \end{tabular*}
% \footnotetext{Note: This is an example of table footnote. This is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
% \footnotetext[1]{Example for a first table footnote.}
% \footnotetext[2]{Example for a second table footnote.}
% \end{minipage}
% \end{center}
% \end{table}

% In case of double column layout, tables which do not fit in single column width should be set to full text width. For this, you need to use \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ instead of \verb+\begin{table}+ \verb+...+ \verb+\end{table}+ environment. Lengthy tables which do not fit in textwidth should be set as rotated table. For this, you need to use \verb+\begin{sidewaystable}+ \verb+...+ \verb+\end{sidewaystable}+ instead of \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ environment. This environment puts tables rotated to single column width. For tables rotated to double column width, use \verb+\begin{sidewaystable*}+ \verb+...+ \verb+\end{sidewaystable*}+.

% \begin{sidewaystable}
% \sidewaystablefn%
% \begin{center}
% \begin{minipage}{\textheight}
% \caption{Tables which are too long to fit, should be written using the ``sidewaystable'' environment as shown here}\label{tab3}
% \begin{tabular*}{\textheight}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
% \toprule%
% & \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]}& \multicolumn{3}{@{}c@{}}{Element\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
% Projectile & Energy	& $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
% \midrule
% Element 3 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
% Element 4 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
% Element 5 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
% Element 6 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
% \botrule
% \end{tabular*}
% \footnotetext{Note: This is an example of table footnote this is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
% \footnotetext[1]{This is an example of table footnote.}
% \end{minipage}
% \end{center}
% \end{sidewaystable}

% \section{Figures}\label{sec6}

% As per the \LaTeX\ standards you need to use eps images for \LaTeX\ compilation and \verb+pdf/jpg/png+ images for \verb+PDFLaTeX+ compilation. This is one of the major difference between \LaTeX\ and \verb+PDFLaTeX+. Each image should be from a single input .eps/vector image file. Avoid using subfigures. The command for inserting images for \LaTeX\ and \verb+PDFLaTeX+ can be generalized. The package used to insert images in \verb+LaTeX/PDFLaTeX+ is the graphicx package. Figures can be inserted via the normal figure environment as shown in the below example:

% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%
% \bigskip
% \begin{verbatim}
% \begin{figure}[<placement-specifier>]
% \centering
% \includegraphics{<eps-file>}
% \caption{<figure-caption>}\label{<figure-label>}
% \end{figure}
% \end{verbatim}
% \bigskip
% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%

% \begin{figure}[h]%
% \centering
% \includegraphics[width=0.9\textwidth]{fig.eps}
% \caption{This is a widefig. This is an example of long caption this is an example of long caption  this is an example of long caption this is an example of long caption}\label{fig1}
% \end{figure}

% In case of double column layout, the above format puts figure captions/images to single column width. To get spanned images, we need to provide \verb+\begin{figure*}+ \verb+...+ \verb+\end{figure*}+.

% For sample purpose, we have included the width of images in the optional argument of \verb+\includegraphics+ tag. Please ignore this. 

% \section{Algorithms, Program codes and Listings}\label{sec7}

% Packages \verb+algorithm+, \verb+algorithmicx+ and \verb+algpseudocode+ are used for setting algorithms in \LaTeX\ using the format:

% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%
% \bigskip
% \begin{verbatim}
% \begin{algorithm}
% \caption{<alg-caption>}\label{<alg-label>}
% \begin{algorithmic}[1]
% . . .
% \end{algorithmic}
% \end{algorithm}
% \end{verbatim}
% \bigskip
% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%

% You may refer above listed package documentations for more details before setting \verb+algorithm+ environment. For program codes, the ``program'' package is required and the command to be used is \verb+\begin{program}+ \verb+...+ \verb+\end{program}+. A fast exponentiation procedure:

% \begin{program}
% \BEGIN \\ %
%   \FOR i:=1 \TO 10 \STEP 1 \DO
%      |expt|(2,i); \\ |newline|() \OD %
% \rcomment{Comments will be set flush to the right margin}
% \WHERE
% \PROC |expt|(x,n) \BODY
%           z:=1;
%           \DO \IF n=0 \THEN \EXIT \FI;
%              \DO \IF |odd|(n) \THEN \EXIT \FI;
% \COMMENT{This is a comment statement};
%                 n:=n/2; x:=x*x \OD;
%              \{ n>0 \};
%              n:=n-1; z:=z*x \OD;
%           |print|(z) \ENDPROC
% \END
% \end{program}


% \begin{algorithm}
% \caption{Calculate $y = x^n$}\label{algo1}
% \begin{algorithmic}[1]
% \Require $n \geq 0 \vee x \neq 0$
% \Ensure $y = x^n$ 
% \State $y \Leftarrow 1$
% \If{$n < 0$}\label{algln2}
%         \State $X \Leftarrow 1 / x$
%         \State $N \Leftarrow -n$
% \Else
%         \State $X \Leftarrow x$
%         \State $N \Leftarrow n$
% \EndIf
% \While{$N \neq 0$}
%         \If{$N$ is even}
%             \State $X \Leftarrow X \times X$
%             \State $N \Leftarrow N / 2$
%         \Else[$N$ is odd]
%             \State $y \Leftarrow y \times X$
%             \State $N \Leftarrow N - 1$
%         \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
% \bigskip
% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%

% Similarly, for \verb+listings+, use the \verb+listings+ package. \verb+\begin{lstlisting}+ \verb+...+ \verb+\end{lstlisting}+ is used to set environments similar to \verb+verbatim+ environment. Refer to the \verb+lstlisting+ package documentation for more details.

% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%
% \bigskip
% \begin{minipage}{\hsize}%
% \lstset{frame=single,framexleftmargin=-1pt,framexrightmargin=-17pt,framesep=12pt,linewidth=0.98\textwidth,language=pascal}% Set your language (you can change the language for each code-block optionally)
% %%% Start your code-block
% \begin{lstlisting}
% for i:=maxint to 0 do
% begin
% { do nothing }
% end;
% Write('Case insensitive ');
% Write('Pascal keywords.');
% \end{lstlisting}
% \end{minipage}

% \section{Cross referencing}\label{sec8}

% Environments such as figure, table, equation and align can have a label
% declared via the \verb+\label{#label}+ command. For figures and table
% environments use the \verb+\label{}+ command inside or just
% below the \verb+\caption{}+ command. You can then use the
% \verb+\ref{#label}+ command to cross-reference them. As an example, consider
% the label declared for Figure~\ref{fig1} which is
% \verb+\label{fig1}+. To cross-reference it, use the command 
% \verb+Figure \ref{fig1}+, for which it comes up as
% ``Figure~\ref{fig1}''. 

% To reference line numbers in an algorithm, consider the label declared for the line number 2 of Algorithm~\ref{algo1} is \verb+\label{algln2}+. To cross-reference it, use the command \verb+\ref{algln2}+ for which it comes up as line~\ref{algln2} of Algorithm~\ref{algo1}.

% \subsection{Details on reference citations}\label{subsec7}

% Standard \LaTeX\ permits only numerical citations. To support both numerical and author-year citations this template uses \verb+natbib+ \LaTeX\ package. For style guidance please refer to the template user manual.

% Here is an example for \verb+\cite{...}+: \cite{bib1}. Another example for \verb+\citep{...}+: \citep{bib2}. For author-year citation mode, \verb+\cite{...}+ prints Jones et al. (1990) and \verb+\citep{...}+ prints (Jones et al., 1990).

% All cited bib entries are printed at the end of this article: \cite{bib3}, \cite{bib4}, \cite{bib5}, \cite{bib6}, \cite{bib7}, \cite{bib8}, \cite{bib9}, \cite{bib10}, \cite{bib11} and \cite{bib12}.

% \section{Examples for theorem like environments}\label{sec10}

% For theorem like environments, we require \verb+amsthm+ package. There are three types of predefined theorem styles exists---\verb+thmstyleone+, \verb+thmstyletwo+ and \verb+thmstylethree+ 

% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%
% \bigskip
% \begin{tabular}{|l|p{19pc}|}
% \hline
% \verb+thmstyleone+ & Numbered, theorem head in bold font and theorem text in italic style \\\hline
% \verb+thmstyletwo+ & Numbered, theorem head in roman font and theorem text in italic style \\\hline
% \verb+thmstylethree+ & Numbered, theorem head in bold font and theorem text in roman style \\\hline
% \end{tabular}
% \bigskip
% %%=============================================%%
% %% For presentation purpose, we have included  %%
% %% \bigskip command. please ignore this.       %%
% %%=============================================%%

% For mathematics journals, theorem styles can be included as shown in the following examples:

% \begin{theorem}[Theorem subhead]\label{thm1}
% Example theorem text. Example theorem text. Example theorem text. Example theorem text. Example theorem text. 
% Example theorem text. Example theorem text. Example theorem text. Example theorem text. Example theorem text. 
% Example theorem text. 
% \end{theorem}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

% \begin{proposition}
% Example proposition text. Example proposition text. Example proposition text. Example proposition text. Example proposition text. 
% Example proposition text. Example proposition text. Example proposition text. Example proposition text. Example proposition text. 
% \end{proposition}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

% \begin{example}
% Phasellus adipiscing semper elit. Proin fermentum massa
% ac quam. Sed diam turpis, molestie vitae, placerat a, molestie nec, leo. Maecenas lacinia. Nam ipsum ligula, eleifend
% at, accumsan nec, suscipit a, ipsum. Morbi blandit ligula feugiat magna. Nunc eleifend consequat lorem. 
% \end{example}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

% \begin{remark}
% Phasellus adipiscing semper elit. Proin fermentum massa
% ac quam. Sed diam turpis, molestie vitae, placerat a, molestie nec, leo. Maecenas lacinia. Nam ipsum ligula, eleifend
% at, accumsan nec, suscipit a, ipsum. Morbi blandit ligula feugiat magna. Nunc eleifend consequat lorem. 
% \end{remark}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

% \begin{definition}[Definition sub head]
% Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. 
% \end{definition}

% Additionally a predefined ``proof'' environment is available: \verb+\begin{proof}+ \verb+...+ \verb+\end{proof}+. This prints a ``Proof'' head in italic font style and the ``body text'' in roman font style with an open square at the end of each proof environment. 

% \begin{proof}
% Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. 
% \end{proof}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

% \begin{proof}[Proof of Theorem~{\upshape\ref{thm1}}]
% Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. 
% \end{proof}

% \noindent
% For a quote environment, use \verb+\begin{quote}...\end{quote}+
% \begin{quote}
% Quoted text example. Aliquam porttitor quam a lacus. Praesent vel arcu ut tortor cursus volutpat. In vitae pede quis diam bibendum placerat. Fusce elementum
% convallis neque. Sed dolor orci, scelerisque ac, dapibus nec, ultricies ut, mi. Duis nec dui quis leo sagittis commodo.
% \end{quote}

% Sample body text. Sample body text. Sample body text. Sample body text. Sample body text (refer Figure~\ref{fig1}). Sample body text. Sample body text. Sample body text (refer Table~\ref{tab3}). 

% \section{Methods}\label{sec11}

% Topical subheadings are allowed. Authors must ensure that their Methods section includes adequate experimental and characterization data necessary for others in the field to reproduce their work. Authors are encouraged to include RIIDs where appropriate. 

% \textbf{Ethical approval declarations} (only required where applicable) Any article reporting experiment/s carried out on (i)~live vertebrate (or higher invertebrates), (ii)~humans or (iii)~human samples must include an unambiguous statement within the methods section that meets the following requirements: 

% \begin{enumerate}[1.]
% \item Approval: a statement which confirms that all experimental protocols were approved by a named institutional and/or licensing committee. Please identify the approving body in the methods section

% \item Accordance: a statement explicitly saying that the methods were carried out in accordance with the relevant guidelines and regulations

% \item Informed consent (for experiments involving humans or human tissue samples): include a statement confirming that informed consent was obtained from all participants and/or their legal guardian/s
% \end{enumerate}

% If your manuscript includes potentially identifying patient/participant information, or if it describes human transplantation research, or if it reports results of a clinical trial then  additional information will be required. Please visit (\url{https://www.nature.com/nature-research/editorial-policies}) for Nature Portfolio journals, (\url{https://www.springer.com/gp/authors-editors/journal-author/journal-author-helpdesk/publishing-ethics/14214}) for Springer Nature journals, or (\url{https://www.biomedcentral.com/getpublished/editorial-policies\#ethics+and+consent}) for BMC.

% \section{Discussion}\label{sec12}

% Discussions should be brief and focused. In some disciplines use of Discussion or `Conclusion' is interchangeable. It is not mandatory to use both. Some journals prefer a section `Results and Discussion' followed by a section `Conclusion'. Please refer to Journal-level guidance for any specific requirements. 

% \section{Conclusion}\label{sec13}

% Conclusions may be used to restate your hypothesis or research question, restate your major findings, explain the relevance and the added value of your work, highlight any limitations of your study, describe future directions for research and recommendations. 

% In some disciplines use of Discussion or 'Conclusion' is interchangeable. It is not mandatory to use both. Please refer to Journal-level guidance for any specific requirements. 

% \backmatter

% \bmhead{Supplementary information}

% If your article has accompanying supplementary file/s please state so here. 

% Authors reporting data from electrophoretic gels and blots should supply the full unprocessed scans for key as part of their Supplementary information. This may be requested by the editorial team/s if it is missing.

% Please refer to Journal-level guidance for any specific requirements.

% \bmhead{Acknowledgments}

% Acknowledgments are not compulsory. Where included they should be brief. Grant or contribution numbers may be acknowledged.

% Please refer to Journal-level guidance for any specific requirements.

% \section*{Declarations}

% Some journals require declarations to be submitted in a standardised format. Please check the Instructions for Authors of the journal to which you are submitting to see if you need to complete this section. If yes, your manuscript must contain the following sections under the heading `Declarations':

% \begin{itemize}
% \item Funding
% \item Conflict of interest/Competing interests (check journal-specific guidelines for which heading to use)
% \item Ethics approval 
% \item Consent to participate
% \item Consent for publication
% \item Availability of data and materials
% \item Code availability 
% \item Authors' contributions
% \end{itemize}

% \noindent
% If any of the sections are not relevant to your manuscript, please include the heading and write `Not applicable' for that section. 

% %%===================================================%%
% %% For presentation purpose, we have included        %%
% %% \bigskip command. please ignore this.             %%
% %%===================================================%%
% \bigskip
% \begin{flushleft}%
% Editorial Policies for:

% \bigskip\noindent
% Springer journals and proceedings: \url{https://www.springer.com/gp/editorial-policies}

% \bigskip\noindent
% Nature Portfolio journals: \url{https://www.nature.com/nature-research/editorial-policies}

% \bigskip\noindent
% \textit{Scientific Reports}: \url{https://www.nature.com/srep/journal-policies/editorial-policies}

% \bigskip\noindent
% BMC journals: \url{https://www.biomedcentral.com/getpublished/editorial-policies}
% \end{flushleft}


==> preamble/acronyms.tex <==

\newacronym{phe}{PHE}{Public Health England}
\newacronym{nhs}{NHS}{National Health Service}
\newacronym{sarscov2}{SARS-CoV-2}{severe acute respiratory syndrome coronavirus 2}
\newacronym{uk}{UK}{United Kingdom}
\newacronym{covid}{COVID-19}{coronavirus disease 2019}
\newacronym{pcr}{PCR}{reverse transcription polymerase chain reaction}
\newacronym{lfd}{LFD}{lateral flow device}
\newacronym{lft}{LFT}{lateral flow test}
\newacronym{npi}{NPI}{non-pharmaceutical intervention}
\newacronym{ons}{ONS}{Office for National Statistics}
\newacronym{cis}{CIS}{COVID-19 Infection Survey}
\newacronym{react}{REACT}{REal-time Assessment of Community Transmission}
\newacronym{dag}{DAG}{directed acyclic graph}
\newacronym[longplural={lower tier local authorities}]{ltla}{LTLA}{lower tier local authority}
\newacronym{eb}{EB}{empirical Bayes}
\newacronym{ci}{CI}{credible interval}
\newacronym{voc}{VoC}{variant of concern}
\newacronym{sgtf}{SGTF}{S gene target failure}
\newacronym{sir}{SIR}{Susceptible-Infectious-Recovered}
\newacronym{dtmc}{DTMC}{discrete time Markov chain}
\newacronym{seir}{SEIR}{Susceptible-Exposed-Infectious-Removed}
\newacronym{si}{SI}{Supplementary Information}
\newacronym{ses}{SES}{socioeconomic status}
\newacronym{ode}{ODE}{ordinary differential equation}
\newacronym{lad}{LAD}{local authority district}
\newacronym{la}{LA}{local authority}
\newacronym{delve}{DELVE}{Data Evaluation and Learning for Viral Epidemics}
\newacronym{cmmid}{cmmid}{centre for mathematical modelling of infectious diseases}
\newacronym{mrc}{MRC}{Medical Research Council}
\newacronym{bsu}{BSU}{Biostatistics Unit}
\newacronym{ct}{CT}{chest computed tomography}
\newacronym{cxr}{CXR}{chest radiograph}
\newacronym{covidpos}{COVID$^{+}$\xspace\unskip}{\gls{sarscov2} \gls{pcr}-positive}
\newacronym{covidneg}{COVID$^{-}$\xspace\unskip}{\gls{sarscov2} \gls{pcr}-negative}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{bnn}{BNN}{Bayesian Neural Network}
\newacronym{ssast}{SSAST}{Self-Supervised Audio Spectrogram Transformer}
\newacronym{mfcc}{MFCCs}{Mel-frequency cepstral coefficients}
\newacronym{uar}{UAR}{Unweighted Average Recall}
\newacronym{roc}{ROC-AUC}{Receiver Operating Charateristic Area Under the Curve}
\newacronym{pr}{PR-AUC}{Precision Recall Area Under the Curve}
\newacronym{mi}{MI}{Mutual Information}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{pc}{PC}{Principal Component}
\newacronym{fdr}{FDR}{False Discovery Rate}
\newacronym{who}{WHO}{World Health Organization}
\newacronym{abcs}{ABCS}{audio-based COVID-19 screening}
\newacronym{eu}{EU}{expected utility}
\newacronym{tt}{T+T}{Test-and-Trace}
\newacronym{rf}{RF}{random forest}
\newacronym{auc}{AUC}{Area Under the Curve}
\newacronym{gdpr}{GDPR}{General Data Protection Regulation}
% \newacronym{ifr}{IFR}{infection fatality ratio}
% \newacronym{iar}{IFR}{infection fatality ratio}
\newacronym{tsne}{t-SNE}{t-distributed stochastic neighbor embedding}
\newacronym{ukhsa}{UKHSA}{UK Health Security Agency}


==> preamble/our_commands.tex <==
\newcommand\ylab{y_i}
\newcommand\xlab{x_i}
\newcommand\predlab{\hat{h}(x_i)}
\newcommand\zlab{z_i}
\newcommand\wlab{w_i}
\newcommand\vlab{v_i}
\newcommand\elab{e_i}
\newcommand{\B}[1]{\boldsymbol{#1}}


==> references/sn-bibliography.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> tables_to_import.tex <==




% \begin{table}[h]
% \begin{center}
% \begin{minipage}{\textwidth}
% \caption{Main Results: Sentence Modality}\label{tab1}%
% \begin{tabularx}{\textwidth}{XX||XXXX||XXXX||X}
% \toprule
%  & Train  & \multicolumn{4}{c||}{Standard}  & \multicolumn{4}{c||}{Matched} & Naive\\
%  \cline{2-11}
%  & Test & Test & Match & Long & Long Match & Test & Match & Long & Long Match & Test \\
% \midrule
%     & UAR & 0.669 & 0.566 & 0.699 & 0.570 & 0.658 & 0.567 & 0.646 & 0.579 & 0.721 \\
% \cline{2-11}
% SVM & ROC & 0.732 & 0.596 & 0.766 & 0.591 & 0.714 & 0.600 & 0.693 & 0.597 & 0.796\\
% \cline{2-11}
%       & PR & 0.578 & 0.574 & 0.625 & 0.580 & 0.553 & 0.583 & 0.515 & 0.576 & 0.686\\
% \midrule
%     & UAR & & & & & & & & & \\
% \cline{2-11}
% BNN       & ROC & & & & & & & & & \\
% \cline{2-11}
%       & PR & & & & & & & & & \\
% \midrule
%       & UAR & 0.733 & 0.594 & 0.739 & 0.583 & 0.691 & 0.602 & 0.666 & 0.572 & 0.763 \\
% \cline{2-11}
% SSAST & ROC & 0.800 & 0.619 & 0.818 & 0.621 & 0.760 & 0.635 & 0.732 & 0.604 & 0.846\\
% \cline{2-11}
%       & PR & 0.684 & 0.594 & 0.715 & 0.594 & 0.631 & 0.626 & 0.590 & 0.579 & 0.774\\
       

% \botrule
% \end{tabularx}

% \end{minipage}
% \end{center}
% \end{table}



% \tabcolsep = 2.0pt
% \begin{table}[h]
% \begin{center}
% \begin{minipage}{\textwidth}
% \caption{Main Results}\label{tab1}%
% \begin{tabularx}{\textwidth}{XXX||XXXX||XXXX||X}
% \specialrule{.2em}{.1em}{.1em}\\
%  && Train  & \multicolumn{4}{c||}{Standard}  & \multicolumn{4}{c||}{Matched} & Naive\\
%  \cline{2-12}
%  Mode && Test & Test & Match & Long & Long Match & Test & Match & Long & Long Match & Test \\
% \specialrule{.2em}{.1em}{.1em}\\
%     && UAR & 0.669 & 0.566 & 0.699 & 0.570 & 0.658 & 0.567 & 0.646 & 0.579 & 0.721 \\
% \cline{3-12}
% &SVM & ROC & 0.732 & 0.596 & 0.766 & 0.591 & 0.714 & 0.600 & 0.693 & 0.597 & 0.796\\
% \cline{3-12}
%       && PR & 0.578 & 0.574 & 0.625 & 0.580 & 0.553 & 0.583 & 0.515 & 0.576 & 0.686\\
% \cline{2-12}
% \multirow{3}{}{Sent-ence}   & & UAR & & & & & & & & & \\
% \cline{3-12}
%  &BNN       & ROC & & & & & & & & & \\
% \cline{3-12}
%       && PR & & & & & & & & & \\
% \cline{2-12}
%      & & UAR & 0.733 & 0.594 & 0.739 & 0.583 & 0.691 & 0.602 & 0.666 & 0.572 & 0.763 \\
% \cline{3-12}
% &SSAST & ROC & 0.800 & 0.619 & 0.818 & 0.621 & 0.760 & 0.635 & 0.732 & 0.604 & 0.846\\
% \cline{3-12}
%       && PR & 0.684 & 0.594 & 0.715 & 0.594 & 0.631 & 0.626 & 0.590 & 0.579 & 0.774\\
% \vspace{1}\\
% \specialrule{.2em}{.1em}{.1em}\\
% \vspace{1}\\
%     && UAR & 0.669 & 0.555 & 0.694 & 0.541 & 0.635 & 0.539 & 0.639 & 0.550 & 0.713 \\
% \cline{3-12}
% &SVM & ROC & 0.727 & 0.568 & 0.759 & 0.558 & 0.684 & 0.560 & 0.688 & 0.569 & 0.782\\
% \cline{3-12}
%       && PR & 0.570 & 0.555 & 0.605 & 0.538 & 0.523 & 0.553 & 0.510 & 0.546 & 0.647\\
% \cline{2-12}
% \multirow{3}{}{Three cough}  & & UAR & & & & & & & & & \\
% \cline{3-12}
%  &BNN       & ROC & & & & & & & & & \\
% \cline{3-12}
%       && PR & & & & & & & & & \\
% \cline{2-12}
%      & & UAR & 0.681 & 0.555 & 0.696 & 0.551 & 0.652 & 0.546 & 0.662 & 0.555 & 0.725 \\
% \cline{3-12}
% &SSAST & ROC & 0.750 & 0.577 & 0.781 & 0.569 & 0.714 & 0.571 & 0.723 & 0.568 & 0.809\\
% \cline{3-12}
%       && PR & 0.607 & 0.553 & 0.648 & 0.552 & 0.563 & 0.557 & 0.561 & 0.557 & 0.701\\
% \vspace{1}\\
% \specialrule{.2em}{.1em}{.1em}\\
% \vspace{1}\\
%  && UAR & 0.648 & 0.536 & 0.685 & 0.540 & 0.633 & 0.541 & 0.638 & 0.538 & 0.695 \\
% \cline{3-12}
% &SVM & ROC & 0.712 & 0.544 & 0.748 & 0.550 & 0.687 & 0.559 & 0.692 & 0.559 & 0.763\\
% \cline{3-12}
%       && PR & 0.559 & 0.526 & 0.594 & 0.535 & 0.533 & 0.550 & 0.521 & 0.545 & 0.625\\
% \cline{2-12}
% & & UAR & & & & & & & & & \\
% \cline{3-12}
% \multirow{3}{}{Cough} &BNN       & ROC & & & & & & & & & \\
% \cline{3-12}
%       && PR & & & & & & & & & \\
% \cline{2-12}
%      & & UAR & 0.681 & 0.545 & 0.690 & 0.541 & 0.638 & 0.528 & 0.640 & 0.543 & 0.702 \\
% \cline{3-12}
% &SSAST & ROC & 0.742 & 0.561 & 0.768 & 0.559 & 0.692 & 0.552 & 0.692 & 0.560 & 0.790\\
% \cline{3-12}
%       && PR & 0.603 & 0.540 & 0.631 & 0.548 & 0.535 & 0.545 & 0.532 & 0.550 & 0.675\\
% \vspace{1}\\
% \specialrule{.2em}{.1em}{.1em}\\
% \vspace{1}\\
%  && UAR & 0.600 & 0.523 & 0.639 & 0.544 & 0.587 & 0.528 & 0.585 & 0.529 & 0.653 \\
% \cline{3-12}
% &SVM & ROC & 0.646 & 0.555 & 0.690 & 0.559 & 0.618 & 0.541 & 0.621 & 0.550 & 0.712\\
% \cline{3-12}
%       && PR & 0.477 & 0.560 & 0.513 & 0.547 & 0.444 & 0.536 & 0.431 & 0.543 & 0.566\\
% \cline{2-12}
% \multirow{3}{}{Ha sound}& & UAR & & & & & & & & & \\
% \cline{3-12}
%  &BNN       & ROC & & & & & & & & & \\
% \cline{3-12}
%       && PR & & & & & & & & & \\
% \cline{2-12}
%      & & UAR & 0.649 & 0.553 & 0.663 & 0.558 & 0.593 & 0.531 & 0.588 & 0.531 & 0.660 \\
% \cline{3-12}
% &SSAST & ROC & 0.701 & 0.581 & 0.725 & 0.580 & 0.653 & 0.552 & 0.644 & 0.556 & 0.750\\
% \cline{3-12}
%       && PR & 0.649 & 0.578 & 0.575 & 0.561 & 0.496 & 0.548 & 0.473 & 0.550 & 0.634\\
% \specialrule{.2em}{.1em}{.1em}\\
% \end{tabularx}

% \end{minipage}
% \end{center}
% \end{table}

